DePIN: A Framework for Token-Incentivized Participatory Sensing

There is always demand for integrating data into microeconomic decision making. Participatory sensing deals with how real-world data may be extracted with stakeholder participation and resolves a problem of Big Data, which is concerned with monetizing data extracted from individuals without their participation. We present how Decentralized Physical Infrastructure Networks (DePINs) extend participatory sensing. We discuss the threat models of these networks and how DePIN cryptoeconomics can advance participatory sensing.

==> name.tex <==
\subsection*{Threat Model and Sensor Node Security}
\label{sec:depin-threat-model-node-sec}

Determining trustworthiness of contributed data is important for both participatory sensing networks as well as DePINs. 
In the case of the latter, the fact that nodes are incentivized for long-term participation implies that they have a higher incentive to act maliciously. Morevover,

discouraging individual nodes from providing malicious data is challenging because it is non-trivial to determine the relationship between quality of the received data stream and potential reward. 
The need to prevent malicious behavior is not restricted to open-hardware use cases since,
although restricting the specific hardware that may register on the network may help with preventing Sybil attacks, the fact remains that a malicious participant may tamper with the environment itself to provide a false, \textit{i.e.}, more beneficial to the participant, sensor reading.


In the following, we describe threats on a per-node basis. 
We begin by defining a DePIN sensor node and, by extension, participatory sensing node.

\paragraph{Sensor Node.}

A sensor node within a DePIN (resp. participatory sensing network) is a physical hardware device 
having the following components:
\begin{enumerate}
\item a processing unit (CPU)
\item writeable memory storage unit (RAM)
\item non-writeable memory (ROM)
\item sensing (measurements) peripherals 
\end{enumerate}

This definition of sensors allows for a broad range of
hardware, ranging from microcontroller-like devices with 
low computational capabilities to more powerful Raspberry Pis,
wherein, in both cases, the peripherals provide sensing or measurement capabilities. There are three main type of threats that sensor nodes face.

\subsubsection*{Device Threats}
Device-level threats include both hardware and software threats. 
Hardware threats are more commonly known as firmware-level threats
since firmware is the crucial low-level piece of software that is responsible
for booting a device or communicating with peripherals (drivers).
It is almost impossible to completely defend against firmware threats during runtime \cite{shah2020survey}
but this concern can be greatly alleviated by strengthening a chain-of-trust \cite{zimmer2016establishing}. 
Software threats are the more traditional and well-known
type of attacks that occur during runtime \cite{or2019dynamic}. In general, software-level
threats are addressed by some form of ``Remote Attestation''. However, 
attestation for less powerful devices such as sensors   are not ideal as they require more power \cite{ammar2020simple} or that the sensor be briefly paused \cite{dushku2020sara}.
We note that, as with all electronics, physical access to hardware
can bypass all firmware and software protections \cite{fu2018}. Hardware approaches to ensuring sensor node security 
either reduce the potential size of the network, by requiring additional functionality such as, for example, 
trusted hardware, or are not sufficient on their own to address the 
threats that a DePIN sensor network face.

\subsubsection*{Network Threats}

Sensors communicate with the broader network over the 
Internet
via APIs. A malicious actor can bypass an actual 
physical device by emulation  
and falsify measurements directly
to the network via the API boundary \cite{wang2018ghost}. 
Note that closed-hardware solutions do not adequately address this class of threats since
they greatly reduce the potential size of the network. 

\subsubsection*{Sensor Environment Threats}

An important class of threats unique to decentralized sensor networks, 
whether classical participatory sensing networks or DePIN sensor 
networks, are attacks where the malicious participant alters the
physical environment of the sensor node or introduces an artificial
element in the sensor node's physical environment. For example, 
a malicious actor can place a sensor at a sub-optimal location for 
measurement in order to record data that might be viewed as %``unique''
and thus 
valuable by the network. Similarly, a malicious actor
can artificially create or modify the sensor environment to achieve the same effect. % so that 

Sensor environment threats are, arguably, the main threats to
DePINs without an adequate way to address 
this type of threat.
